Make the U in UDA Matter: Invariant Consistency Learning for Unsupervised Domain Adaptation

Domain Adaptation (DA) is always challenged by the spurious correlation between domain-invariant features (e.g., class identity) and domain-specific features (e.g., environment) that does not generalize to the target domain. Unfortunately, even enriched with additional unsupervised target domains, existing Unsupervised DA (UDA) methods still suffer from it. This is because the source domain supervision only considers the target domain samples as auxiliary data (e.g., by pseudo-labeling), yet the inherent distribution in the target domain -- where the valuable de-correlation clues hide -- is disregarded. We propose to make the U in UDA matter by giving equal status to the two domains. Specifically, we learn an invariant classifier whose prediction is simultaneously consistent with the labels in the source domain and clusters in the target domain, hence the spurious correlation inconsistent in the target domain is removed. We dub our approach "Invariant CONsistency learning" (ICON). Extensive experiments show that ICON achieves the state-of-the-art performance on the classic UDA benchmarks: Office-Home and VisDA-2017, and outperforms all the conventional methods on the challenging WILDS 2.0 benchmark. Codes are in https://github.com/yue-zhongqi/ICON.

==> A_limitation.tex <==
\section{Limitation and Broader Impact}
\label{sec:A}


\noindent\textbf{Limitation}. Our approach relies on the assumptions in Section 4, \ie, the classes in $T$ are separated by clusters, and there is enough diversity in $T$ such that causal feature $\mathbf{c}$ is the only invariance. We highlight that this is akin to the clustering assumption in semi-supervised learning, which serves as the cornerstone to learning from the unlabeled samples. To further fulfill the assumptions, one could seek additional prior knowledge to highlight the causal feature, \eg, designing improved augmentations that remove more environmental features, leveraging additional pre-trained knowledge from foundation models or improved clustering algorithm.

\noindent\textbf{Broader Impact}. Our work aims to capture the causal feature in the unsupervised domain adaptation setting. In particular, we significantly improve the state-of-the-art on WILDS 2.0 benchmark, which includes practical tasks that benefit wildlife preservation, tumour classification in healthcare, remote sensing, vision in agriculture, \etc. The pursue of causal feature can
produce more robust, transparent and explainable models, broadening the applicability of ML models
and promoting fairness in AI.

==> figures/fig6.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-4mm}
    \centering
    \scriptsize
    \includegraphics[width=\linewidth]{figures/figure6.pdf}
    \caption{(a) Solid lines: test accuracy against training epochs for \textcolor{icongreen}{FixMatch}, \textcolor{iconblue}{CST} and \textcolor{red}{ICON}. Dotted black lines: average loss in each epoch with matching markers to denote the three methods. (b) Among the feature pairs where $f$ fails, the percentage of pairs where $g$ succeeds for the three methods in each epoch.}
    \vspace*{-4mm}
    \label{fig:6}
\end{wrapfigure}

==> figures/proof.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-8mm}
\captionsetup{font=footnotesize,labelfont=footnotesize}
    \centering
    \includegraphics[width=.9\linewidth]{figures/proof.pdf}
    
    \caption{The PDFs of $q(\mathbf{x}_t|\mathbf{x}_0)$ (green) and $q(\mathbf{y}_t|\mathbf{y}_0)$ (blue). Without loss of generality, we consider the 1-D case of $y_0 > x_0$. Their means are computed from Eq. (2).}
    \label{fig:3}
    \vspace{-8mm}
\end{wrapfigure}

==> tables/table2.tex <==
\begin{table}[t!]
\centering
% \captionsetup{font=footnotesize,labelfont=footnotesize,skip=5pt}
\scalebox{0.8}{
\begin{tabular}{p{4 cm} p{2.4cm}<{\centering}p{2.2cm}<{\centering}}
%{cl|cccccc|cccccc}
\hline\hline
\multicolumn{1}{c}{\textbf{Method}} & \textbf{\textsc{Office-Home}} & \textbf{\textsc{VisDA-2017}}\\
\hline
ICON & 75.8 & 87.4 \\
ICON$-$INV & 74.2 & 84.2 \\
ICON$-$INV$-$UMAP & 74.1 & 82.0 \\
Cluster with 2$\times$\#classes & 69.7 & 78.6 \\
Cluster with 0.5$\times$\#classes & 67.5 & 76.2 \\
\hline \hline
\end{tabular}}
\scriptsize
\caption{Ablations on each ICON component.}
\label{tab:2}
\vspace*{-6mm}
\end{table}

==> tables/table_vi.tex <==
\begin{table}[t!]
\centering
% \captionsetup{font=footnotesize,labelfont=footnotesize,skip=5pt}
\scalebox{0.85}{
\begin{tabular}{p{3.6 cm}<{\centering} p{1.8cm} p{3.0cm}<{\centering}}
%{cl|cccccc|cccccc}
\hline\hline
\textbf{Method} & \textbf{Backbone} & \textbf{Mean-Class Acc.}\\
\hline

MT+16augs~\cite{french2017self} (2018) & ResNet-50 & 82.8 \\

MDD~\cite{zhang2019bridging} (2019) & ResNet-50 & 77.8 \\

GVB~\cite{cui2020gradually} (2020) & ResNet-50 & 75.3 \\

TCM~\cite{yue2021transporting} (2021) & ResNet-50 & 75.8 \\

SENTRY~\cite{prabhu2021sentry} (2021) & ResNet-50 & 76.7 \\

CST~\cite{liu2021cycle} (2021) & ResNet-50 & 80.6 \\

CAN$^*$~\cite{kang2019contrastive} (2019) & ResNet-101 & 87.2 \\

SHOT~\cite{liang2020we} (2020) & ResNet-101 & 82.9 \\

FixBi$^*$~\cite{kang2019contrastive} (2021) & ResNet-101 & 87.2 \\

MCC+NWD~\cite{chen2022reusing} (2022) & ResNet-101 & 83.7 \\

SDAC~\cite{rangwani2022closer} (2022) & ResNet-101 & 84.3 \\

kSHOT$^*$~\cite{sun2022prior} (2022) & ResNet-101 & 86.1 \\

\hline

\textbf{ICON (Ours)} & \cellcolor{mygray} ResNet-50 & \cellcolor{mygray}\textbf{87.4} \\

\hline \hline
\end{tabular}}
%\scriptsize
\vspace*{+2mm}
\caption{More results on \textsc{VisDA-2017} supplementary to Table 1. Details on $^*$ in the text. Published years are in the brackets after the method names.}

\label{tab:vi}

\end{table}

% kshot use prior knolwedge on the percentage of samples belonging to each class
